On Learning Meaningful Code Changes via Neural Machine Translation

Recent years have seen the rise of Deep Learning (DL) techniques applied to source code. Researchers have exploited DL to automate several development and maintenance tasks, such as writing commit messages, generating comments and detecting vulnerabilities among others. One of the long lasting dreams of applying DL to source code is the possibility to automate non-trivial coding activities. While some steps in this direction have been taken (e.g., learning how to fix bugs), there is still a glaring lack of empirical evidence on the types of code changes that can be learned and automatically applied by DL. Our goal is to make this first important step by quantitatively and qualitatively investigating the ability of a Neural Machine Translation (NMT) model to learn how to automatically apply code changes implemented by developers during pull requests. We train and experiment with the NMT model on a set of 236k pairs of code components before and after the implementation of the changes provided in the pull requests. We show that, when applied in a narrow enough context (i.e., small/medium-sized pairs of methods before/after the pull request changes), NMT can automatically replicate the changes implemented by developers during pull requests in up to 36% of the cases. Moreover, our qualitative analysis shows that the model is capable of learning and replicating a wide variety of meaningful code changes, especially refactorings and bug-fixing activities. Our results pave the way for novel research in the area of DL on code, such as the automatic learning and applications of refactoring.

==> learning-code-review/intro_copy.tex <==
Code Review is the process of analyzing source code written by a teammate to judge whether it is of sufficient quality to be integrated into the main code trunk. Recent studies provided evidence that reviewed code has lower chances of being buggy \cite{McIntosh:msr2014,morales2015saner,Bavota:icsme2015} and exhibit higher internal quality \cite{Bavota:icsme2015}, likely being easier to comprehend and maintain. Given these obvious benefits, code reviews are widely adopted both in industrial and open source projects with the goal of finding defects, improving code quality, and identifying alternative solutions. 

The benefits brought by code reviews do not come for free. Indeed, code reviews add additional expenses to the standard development costs due to the allocation of one or more reviewers having the responsibility of verifying the correctness, quality, and soundness of newly developed code. Bosu and Carver report that developers spend, on average, more than six hours per week reviewing code \cite{Bosu:2013}. This is not surprising considering the high number of code changes reviewed in some projects: Rigby and Bird \cite{Rigby:fse2013} show that industrial projects such as Microsoft Bing can undergo thousands of code reviews per moth ($\sim$3k in the case of Bing). Also, as recently highlighted by Czerwonka \etal \cite{Czerwonka:icse2015}, the effort spent in code review does not only represent a cost in terms of time, but also pushes developers to switch context from their tasks. \MICHELE{Great motivations! Is anywhere reported in some papers the number of developers assigned for a single code review? Here in my team at Microsoft, any code review needs at least 3 other developers (excluding the original one). I could ask here at Microsoft what are the rules also for other teams, but not sure if we can add this as an anecdotal, or we need a paper citation.}\DENYS{Michele, yes, it would be great if we could cite their technical report, a paper or any other mention on their web-site}

Our long term goal is to reduce the cost of code reviewing by (partially) automating this time-consuming process. Indeed, we believe that several code review activities can be automated, such as, catching bugs, improving adherence to the project's coding style, and refactoring suboptimal design decisions. The final goal is not to replace developers in code review, but to automatically solve (or suggest) code quality issues that developers would manually catch and fix in their final checks. 

In this paper, we make a first step in this direction by presenting \approach, the first approach in the literature learning from real code review activities performed by software developers and able to perform code transformations for a given code under review as developers would do. We harness the power of Neural-Machine Translation (NMT) to automatically ``translate'' the code submitted for review into the code that would be the output of a review process performed by developers, thereby emulating the combination of code changes they would suggest while reviewing. Note that in its current version,  \approach performs the code transformation without providing a rationale for the recommended code changes (\ie it does not emulate the comments posted by reviewers during code review activities). Simulating comments posted by reviewers is out of the scope of this paper, and part of our research agenda.

We mine three large Gerrit \cite{Gerrit} code review repositories, namely Android \cite{gerrit-android}, Google Source \cite{gerrit-google}, and Ovirt \cite{gerrit-ovirt}. In total, these repositories host code reviews related to \textcolor{red}{XXX} sub-projects. We collected from them \textcolor{red}{XXX} merged changes that underwent code review. We only considered merged changes since this allows us to collect, for each reviewed change, the code pre- (\ie submitted for review) and post- (\ie merged) review. We extract from these pairs method-level AST edit operations using fine-grained source code differencing \cite{Falleri:ase2014}. This resulted in \textcolor{red}{XXX} method pairs, each of them representing the method at the beginning and at the end of the review process. An Encoder-Decoder Recurrent Neural Network \cite{} is then used to learn the code transformations performed by developers during code review activities. Once the model has been trained, it is used to automatically review previously unseen code. \approach is also able to propose alternative code transformations for given code under review by employing beam search \cite{}.

We quantitatively and qualitatively evaluate \approach. For the quantitative analysis, we assessed the ability of \approach in modifying the code submitted for review exactly as done by developers during real code review activities. This means that we compare, for the same code submitted for review, the output of the manual code review process and of \approach. The qualitative analysis aims instead at distilling a taxonomy of meaningful code transformations that \approach was able to automatically learn from the training data (\eg which types of refactoring operations it injects, which types of bugs it is able to catch and fix) --- see \figref{fig:taxonomy}.

The achieved results indicate that, in its best configuration, \approach is able to inject the same code transformations that are implemented by developers during code review in 16-36\% of cases, depending from the number of possible solutions \approach is required to produce with the beam search (\eg if only pick the top-ranked solution, \approach succeeds in 16\% of cases). Moreover, the extracted taxonomy shows that \approach is able to learn a rich variety of meaningful code transformations, automatically fixing bugs and refactoring code as humans would do during reviewing activities. Despite somewhat limited performance, we believe that \approach can pave the way to more research targeting the automation of code review. To foster research in this direction, we make publicly available the complete datasets, source code, tools, and raw data used in our experiments \cite{replication}.

==> learning-code-review/related_copy.tex <==
\subsection{Deep Learning in Software Engineering}

\subsection{Deep Learning}
Deep Learning (DL) has recently become a useful way to study different facets of software engineering. The unique representations allow for features to be discovered by the model rather than manual derivation. Due to the power of these representations, many works have applied these models to solve software engineering problems. However, to the best of our knowledge, this is the first work that uses DL techniques to learn and perform code review changes in attempts to automate the source code review process. We continue this section by mentioning works that use DL to solve software engineering problems. 

White \etal uses representation learning via a recursive autoencoder for the task of clone detection \cite{White:2016:DLC:2970276.2970326}. In their work, each piece of source is represented as a stream of identifiers and literals, which they use as input to their DL model. Using a similar encoding, Tufano \etal encodes methods into four different representations; then the DL model evaluates how similar two pieces of source code are based on their multiple representations \cite{Tufano:2018:DLS:3196398.3196431}. These works are similar to ours since we use a similar code representation as input to the DL model, however, we apply this methodology to help automate the code review process. 

White \etal also compares DL models with natural language processing models for the task of code suggestion. They show that DL models and make code suggestions based upon contextual features learned by the model rather than the predictive power of the past “n” tokens \cite{White:2015:TDL:2820518.2820559}. Further expanding upon the powerful, predictive capabilities of these models, Dam \etal presents DeepSoft. DeepSoft is a DL based architecture that is used for modeling software, code generation and software risk prediction \cite{Dam:2016:DVD:2950290.2983985}. 

DL has also been applied to the areas of bug triaging and bug localization. Lam \etal makes use of DL models and information retrieval to localize buggy files for developers after they have received a bug report. They use a revised Vector Space Model to create a representation the DL model can use to relate terms in a bug report to source code tokens \cite{7372035}. Likewise, to reduce the effort of bug triaging, Lee \etal applies a convolutional neural network to industrial software projects in order to properly triage bugs.  This approach uses word2vec to embed a summary and a description which the CNN then assigns to a developer
\cite{Lee:2017:ADL:3106237.3117776}. Related to software bugs, Wang \etal uses a Deep Belief Network (DBN) to automatically learn semantic features from token vectors taken from a programs’ Abstract Syntax Tree (ASTs). The network then predicts if the commit will be defective \cite{Wang:2016:ALS:2884781.2884804}.

Many DL uses are aimed toward helping developers with tasks outside of writing source code. Choetkiertikul \etal proposes a DL architecture of long short-term memory and recurring highway network that aims to predict the effort estimation of a coding task \cite{8255666}. Another aid for developers is the ability to summarize a given segment of source code. To this point Allamanis \etal uses an Attentional Neural Network (ANN) with a convoluation layer in order to summarize pieces of source code into short, functional descriptions \cite{DBLP:journals/corr/AllamanisPS16}. Guo \etal develops a DL approach using recurrent neural networks (RNNs) and word embeddings to learn the sentence semantics of requirement artifacts, this helps to create traceability links in software projects \cite{Guo:2017:SES:3097368.3097370}. The last example of DL implementations that aid developers in the software development process is an approach developed by Gu \etal that helps to locate source code. This implementation uses Neural Networks and natural language to embed code snippets with natural language descriptions into a high-dimensional vector space, this helps developers locate source code based on natural language queries \cite{Gu:2018:DCS:3180155.3180167}.   

DL based approaches have also been applied to more coding related tasks, one such task is accurate method and class naming.  Allamanis \etal uses a log-bilinear neural network to understand the context of a method or class and recommends a representative name that has not appeared in the training corpus \cite{Allamanis:2015:SAM:2786805.2786849}. Also helping with correct coding practices, Gu \etal uses an RNN encoder-decoder model to generate a series of correct API usages in source code based upon natural language queries. The learned semantics allow the model to associate natural language queries with a sequence of API usages \cite{Gu:2016:DAL:2950290.2950334}.

Recently we have seen DL infiltrate the mobile software engineering realm. Moran \etal uses a DL based approach to automatically generate graphical user interfaces for mobile applications. In this approach, a deep convolutional neural network is used to help classify GUI components which can later be used to generate a mock GUI for a specific application \cite {DBLP:journals/corr/abs-1802-02312}.

Although DL approaches are prevalent in software engineering, this work is the first to apply DL to code review tasks that help automate the process for developers. The previous work has shown that DL approaches can yield meaningful results given enough, quality training data. Thus, we apply DL here to automatically learn features of embedded source code and code review actions. We can then use a trained model to predict meaningful code review actions on an unseen piece of source code.

\subsection{Code Review}
Several studies have focused on code review, investigating its impact on the code quality \cite{Kemerer:tse2009,morales2015saner,McIntosh:msr2014,Bavota:icsme2015}. Kemerer and Paulk \cite{Kemerer:tse2009}, McIntosh \etal \cite{McIntosh:msr2014}, and Bavota and Russo \cite{Bavota:icsme2015} agree in reporting the lower likelihood of introducing bugs in reviewed code as compared to non-reviewed code. Also, Morales \etal \cite{morales2015saner} and Bavota and Russo \cite{Bavota:icsme2015} confirm the higher code quality ensured by code review. 

Other authors studied how the code review process is carried out in industry and in open source communities \cite{Rigby:icse2008,Rigby:icse2011,Bacchelli:icse2013,Bosu:2013,Rigby:fse2013,BellerEtAl:2014,Czerwonka:icse2015,Kononenko:icse2016,Bosu:tse2017}. Due to space constraints, we do not discuss these works in details but we only summarize some of the findings relevant for our work. Identifying defects has been confirmed in different studies \cite{Rigby:icse2008,Bacchelli:icse2013,BellerEtAl:2014,Bosu:tse2017} as the main reason for performing code review, thus highlighting the importance of automating this activity. These studies also provided evidence of the substantial time invested in code review activities \cite{Bosu:2013,Rigby:fse2013,Czerwonka:icse2015}, one of the motivations for working on code review automation.

Researchers also analyzed the factors influencing the acceptance of the code changes submitted for review \cite{WeiBgerber:2008,Baysal:wcre2013,BosuCarver:2014A,BosuCarver:2014B}. They found that (i) smaller changes have a higher chance to be accepted \cite{WeiBgerber:2008}, and (ii) non-technical factors such as the experience of the developer submitting the change influences the review outcome \cite{Baysal:wcre2013,BosuCarver:2014A,BosuCarver:2014B}.

Finally, a recent work proposed a tool, named ClusterChanges, to help developers during the code review process \cite{Barnett:icse2015}. This is certainly the work more related to ours. However, while the overall goal (\ie helping developers during code review) is the same, two different problems are tackled by ClusterChanges and \approach. ClusterChanges automatically decomposes changesets submitted for review into cohesive, smaller changes, with the goal of simplify the code review process. \approach, instead, can be used to automatically transform the code submitted for review into the one likely resulting from a manual code review (with all limitations we discussed). In future, we plan to investigate the combination of these two techniques. Indeed, we believe that ClusterChanges could be use in improved versions of \approach that will learn not by pairs of methods, but by the whole code (\eg the whole files) pre- and post-review. In this scenario, ClusterChanges would allow to train \approach on more cohesive changesets.
